A Large-Scale Study of the Twitter Follower Network to Characterize the Spread of Prescription Drug Abuse Tweets

In this article, we perform a large-scale study of the Twitter follower network, involving around 0.42 million users who justify DA, to characterize the spreading of DA tweets across the network. Our observations reveal the existence of a very large giant component involving 99% of these users with dense local connectivity that facilitates the spreading of such messages. We further identify active cascades over the network and observe that the cascades of DA tweets get spread over a long distance through the engagement of several closely connected groups of users. Moreover, our observations also reveal a collective phenomenon, involving a large set of active fringe nodes (with a small number of follower and following) along with a small set of well-connected nonfringe nodes that work together toward such spread, thus potentially complicating the process of arresting such cascades. Furthermore, we discovered that the engagement of the users with respect to certain drugs, such as Vicodin, Percocet, and OxyContin, that were observed to be most mentioned in Twitter is instantaneous. On the other hand, for drugs, such as Lortab, that found lesser mentions, the engagement probability becomes high with increasing exposure to such tweets, thereby indicating that drug abusers engaged on Twitter remain vulnerable to adopting newer drugs, aggravating the problem further.

==> sections/PDAN_Characteristics.tex <==
\section{Characterizing PDAN}
\label{sec:PDAN_Characteristics}
% \begin{table}
% \centering
% \begin{tabular}{ |l|c| } 
%  \hline
%   Network Property & Value \\
%   \hline
%   Number of Nodes  & $278,448$  \\
%   Number of links & $4,966,424$\\
%   Average (in/out) degree & $ 19.05$   \\
%   In-degree slope & $-1.51$   \\
%   Out-degree slope & $-2.00$   \\
%   Number of Component & $384$\\
%   Giant Component Size  & $259,623$ \\
%   Clustering coefficient & $0.1479$\\
%   Reciprocity & $ 0.6182$\\
%   \hline
% \end{tabular}
% \caption{Statistics of Prescription Drug Abuse Network.}
% \label{tab:PDAN_Stat}
% \end{table}
We highlight some of the major network properties of PDAN (summarized in table~\ref{tab:PDAN_Stat}) that would impact spreading in the network. 
\subsubsection*{Basic Statistics:} We observe that there exists a large prescription abuse network consisting of approximately $0.28$ million unique users with $0.5$ million links between them. The number of followers (in-degree) and followings (out-degree) of the nodes in PDAN follow power-law distributions with exponents $1.48$ and $2.05$, respectively. Figure~\ref{fig:network_stats}\subref{fig:follower_following-dis}, shows the complementary cumulative distribution (CCDF) of the number of  followers and followings within the PDAN. It may be noted that the observed exponent for the in-degree observed is much lower as compared to the entire Twitter network ($2.276$, as reported in~\cite{kwak2010twitter}). This indicates that a significant fraction of drug abusers have a very high number of followers ($42\%$ users have more than $10$  followers and $2\%$, i.e. 6,109 users, have more than $100$ followers in PDAN), suggesting the possibility of a significant spread of the drug abuse tweets if suitable connections exist among the nodes across the PDAN. Consequently, we observe three major structural properties of the PDAN --- the connectedness among the nodes, the average clustering coefficient and the reciprocity of the links --- all of which play important role in the spread of tweets and can subsequently impact the user engagement.
\begin{table}[!htb]
\centering
\footnotesize
\begin{tabular}{ |l|c| } 
 \hline
  Network Property & Value \\
  \hline
  Number of Nodes  & $278,448$  \\
  Number of links & $4,966,424$\\
  Average (in/out) degree & $ 19.05$   \\
  In-degree slope & $-1.51$   \\
  Out-degree slope & $-2.00$   \\
  Number of Component & $384$\\
  Giant Component Size  & $259,623$ \\
  Clustering coefficient & $0.1479$\\
  Reciprocity & $ 0.6182$\\
  \hline
\end{tabular}
\caption{Statistics of Prescription Drug Abuse Network.}
\label{tab:PDAN_Stat}
\end{table}

% \begin{figure}
% \subfloat[Out-degree distribution of PDAN.\label{fig:out-deg}]{%
%   \includegraphics[width=1.5 in]{out_degree.pdf}%
% }\hfill
% \subfloat[In-degree distribution of PDAN.\label{fig:in-deg}]{%
%   \includegraphics[width=1.5 in]{in_degree.pdf}%
% }\hfill
% % \subfloat[Percentage of Population of drug abuser of different age group\label{fig:age_drug_abuser}]{%
% %   \includegraphics[height=2.1 in, width=.33\linewidth]{age_drug_abuser}%
% %   }
% \caption{Distribution of the out-degree and in-degree of users in PDAN. In figure \ref{fig:out-deg}, we plot the probability of occurrence (in log scale ) of along y-axis and out-degree of a node (in log scale ) along the x-axis. Similarly, we plot in-degree of a node (in log scale ) along x-axis and probability of occurrence (in log scale ) along the y-axis in figure \ref{fig:in-deg}.}
% \label{fig:PDAN_stat}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=2.5 in]{ccdf_degree.pdf}
% \caption{Number of followings and followers. 
% %\textcolor{red}{sourav:which figure shows what? not clear.}
% }
% \label{fig:follower_following_dis}
% \end{figure}


\begin{figure}
\subfloat[CCDF of followings and followers. \label{fig:follower_following-dis}]{%
  \includegraphics[width=0.22\textwidth]{images/ccdf_degree.pdf}%
} \hspace{0.2in}
\subfloat[CCDF of number of tweets of users in PDAN. \label{fig:tweet-dis}]{%
  \includegraphics[width=0.22\textwidth]{images/ccdf_tweets_distr.pdf}%
} 
%\hspace{0.2in}
%\subfloat[Schematic diagram of a Bowtie. \label{fig:bowtie}]{%
%  \includegraphics[width=0.45\textwidth]{images/bowtie.pdf}%
%}
% \subfloat[Percentage of Population of drug abuser of different age group\label{fig:age_drug_abuser}]{%
%   \includegraphics[height=2.1 in, width=.33\linewidth]{age_drug_abuser}%
%   }
\caption{~\protect\subref{fig:follower_following-dis} represents CCDF of the follower count and following count of the users and ~\protect\subref{fig:tweet-dis} represents CCDF of the number of tweets of users in the network. 
%~\protect\subref{fig:bowtie} pictorially represents the bowtie structure of PDAN.
} 
\label{fig:network_stats}
\end{figure}


% \begin{figure}[h]
% \centering     %%% not \center
% \subfigure[Distribution of number of tweets of PDAN.]{\label{fig:tweet_dis}\includegraphics[width=1.5 in]{tweet_dis_U}}
% \subfigure[Distribution of follower count of PDAN.]{\label{fig:follower_dis}\includegraphics[width=1.5 in]{follower_dis_U}}
% %\subfigure[Distribution of personalized influence score .]{\label{fig:PI_dis}\includegraphics[width=1.75 in, height=1.58in]{images/PI_dis}}
% \caption{Distribution of the number of tweets and follower count of users in PDAN. In figure \ref{fig:tweet_dis}, we plot the probability of occurrence (in log scale ) of along y-axis and number of tweets of a node (in log scale ) along the x-axis. Similarly, we plot number of the follower (in log scale ) along x-axis and probability of occurrence (in log scale ) along the y-axis in figure \ref{fig:follower_dis}. }
% \label{fig:PDAN_stat}
% \end{figure}
%%%JC On an average the users in PDAN have around $2,081$ followers (including the followers who are not in PDAN) and follow around $680$ user {which indicates they are popular users}. 
%\ToDo{Also explicitly mention how much percentage of users have less than 10 followers - is it 50\%??}\Reply{JC: Ryan update - Done}
\subsubsection*{Connectedness:} We observe that although there are $384$ components in the network, the size of the giant component is $93.24\%$ of the whole PDAN with $259,623$ nodes. But the second and the third largest connected components have 107 and 28 nodes respectively, and there exist several smaller components with an average size of around $3$. %\todo{What is the size of the second largest component?} 
 %It is further observed\blue{, in table \ref{tab:bowtie},} that the PDAN emerges as a 
 Further, if  we model the (giant component) network as a BowTie structure~\cite{broder2000graph} 
 %(Figure~\ref{fig:network_stats}\subref{fig:bowtie}) 
 it is found that  around $87\%$ of the nodes (refer table \ref{tab:bowtie}) fall in the largest connected component (LSCC) or the core of the structure with much fewer node in the IN and OUT components.
%%%JC The percentage of IN nodes, i.e. the ones that are following one or more nodes in the core is around $10\%$ whereas the corresponding OUT percentage is around $1.5\%$. A minuscule of the nodes are TENDRIL nodes ($1\%$), with no direct connectivity to the core nodes. The bow-tie connection often determines the resilience and robustness of the system. 
A large core, apart from being resilient to targeted attacks, also implies the possibility of faster diffusion of drug abuse tweets over a large fraction of the network~\cite{blackJTB1966}. %\ToDo{The people in this community may not be too aware of bow-tie structure, we have to also explain its implication.}\Reply{JC: Done, Pls see}
\begin{table}[!htb]
\centering
\footnotesize
\begin{tabular}{|l|c|c|}
\hline
Component&Count&Percentage\\
\hline
LSCC&226,254&86.77\\
IN&26,606&10.20\\
OUT&3,917&1.50\\
Tendrils&2,846&1.09\\
%Disconnected&1,124&0.43\\
\hline
\end{tabular}
\caption{Distribution of users of giant component in different Bowtie components.}
\label{tab:bowtie}
\end{table}

 
 \subsubsection*{Clustering Coefficient: } The undirected PDAN exhibits a high average clustering coefficient of around $0.15$ that is significantly higher than observed in the actual Twitter network ($0.096$)~\cite{AparicioEntropy15}. Although a high clustering coefficient has generally been considered as an impediment to large scale diffusion across the networks~\cite{peresPhysica2014}, however, nodes within a closely connected cluster can get entrapped in the echo chambers, where they persistently receive only those tweets that glorify drug abuse~\cite{garimellaWWW2018}. 
 %%%%JC \ToDo{This is an important point Sourav pointed out - can this be connected with the cascade formation - what is the clustering coefficent of each cacades - are they much higher than 0.15} \Reply{The clustering coefficient of cascades is 0 as its a tree like structure.}
%\todo{This is a directed network, CC in directed networks are not well defined, how are you finding this? Rather you should highlight the core periphery structure, like the bow ties structure}
\subsubsection*{Reciprocity: } Our investigation further reveals the existence of a very high reciprocity ($62\%$ of total links) in the network. This value is significantly higher than the reciprocity value of around 22\% observed in the Twitter follower-followee network studied in ~\cite{kwak2010twitter}. Previous studies have indicated that the existence of high reciprocal links not only affects the coverage of the spread of messages in social networks but also enhances the speed of the diffusion~\cite{zhu2014influence}.
\par \textcolor{red}{Surprisingly, all these characteristics are consistent with several other networks, where behavioral spreading has been observed~\cite{centolaScience2010}. We later investigate the impact of these structural properties of the PDAN on the cascades. However, these statistics point towards the existence of an underlying network platform that is amenable to the spread of the drug abuse tweets by an active engagement of a set of users. Hence we next attempt to characterize the users in  the PDAN by their engagement pattern. } 
%The high reciprocity also indicates the possibility of the nodes to gain influence by farming new links~\cite{ghosh2012understanding}. 
%JC The large giant component indicates the capability of the network to spread promotional tweets to a very large fraction of users. We also observe the follower and following count of the users in the network. Figure~\ref{fig:follower_following-dis}, shows the complementary cumulative distribution function (CCDF) of the follower and following count of users in PDAN. The graph indicates that a significant fraction of drug abusers have a very high number of follower and following count. This indicates that certain users do have the capability of reaching out to a large fraction of users and hence can play a dominant role in the spread of drug abuse. 
%%%JC \par We next investigate the characteristics of the user's activities and their role in the PDAN.

% \begin{figure}[h]
% \centering
% \includegraphics[width=2.5 in]{tweets_distr.pdf}
% \caption{Frequency distribution of the number of tweets posted by each user in PDAN. 
% %\textcolor{red}{sourav:which figure shows what? not clear.}
% }
% \label{fig:tweet-dis}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=2.5 in]{ccdf_tweets_distr.pdf}
% \caption{Complementary Cumulative Distribution Function (CCDF) of number of tweets of users in PDAN. 
% %\textcolor{red}{sourav:which figure shows what? not clear.}
% }
% \label{fig:tweet-dis}
% \end{figure}




% \begin{figure}
% \subfloat[\label{fig:followers_vs_following} follower count vs. following count]{%
%   \includegraphics[width=1.6 in]{followers_vs_following.pdf}%
% }\hfill
% \subfloat[\label{fig:followers_vs_tweets}Follower count vs. average number of tweets of user]{%
%   \includegraphics[width=1.6 in]{followers_vs_tweets.pdf}%
% }\hfill
% \caption{Figure \subref{fig:followers_vs_following} represents along x-axis, the number of followers of user and along y-axis, it represents following count. In figure  \subref{fig:followers_vs_tweets}, it represents the average number of tweets along y-axis and along x-axis,it represents number of follower.}
% \label{fig:followers_stats}
% \end{figure}
